Validation of HD 183579b using archival radial velocities: a warm-neptune orbiting a bright solar analog

As exoplanetary science matures into its third decade, we are increasingly offered the possibility of pre existing, archival observations for newly detected candidates. This is particularly poignant for the TESS mission, whose survey spans bright, nearby dwarf stars in both hemispheres, which are precisely the types of sources targeted by previous radial velocity (RV) surveys. On this basis, we investigated whether any of the TESS Objects of Interest (TOIs) coincided with such observations, from which we find 18 single planet candidate systems. Of these, one exhibits an RV signature that has the correct period and phase matching the transiting planetary candidate with a false alarm probability of less than 1 percent. After further checks, we exploit this fact to validate HD 183579b (TOI-1055b). This planet is less than 4 Earth Radii and has better than 33 percent planetary mass measurements, thus advancing the TESS primary objective of finding 50 such worlds. We find that this planet is amongst the most accessible small transiting planets for atmospheric characterization. Our work highlights that the efforts to confirm and even precisely measure the masses of new transiting planet candidates need not always depend on acquiring new observations - that in some instances these tasks can be completed with existing data.

==> modeltable.tex <==
\begin{table*}
\caption{
Statistical tests for evidence for exomoons, using gravitational effects only.
Answers to the three questions posed at the start of Section~\ref{sec:analysis}
are provided in columns 2, 3 \& 4, where the first number denotes the statistic
used to assess each question, and the mark in square brackets is a simple yes/no
summary of the posed question. The final column gives a mass ratio upper limit
derived.
%
We also show the same tests for Kepler-1625b \citep{teachey:2018}, although the
cross-validation test is not possible due to the limited number of samples, and
a mass upper limit is not provided since this case corresponds to a detection.
%
} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c c} % centered columns (8 columns)
\hline\hline %inserts double horizontal lines
KOI &
$\mathrm{BIC}_{\mathcal{P}-\mathcal{T})}$ \textbf{[Q1]} &
\% of good TTV predictions \textbf{[Q2]} &
$\log K_{\mathcal{M}:\mathcal{X}}$ \textbf{[Q3]} &
$(M_S/M_P)$ at 60\,$R_P$ [2$\sigma$]\\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
268.01	& $-31.0$ [\text{\sffamily X}]	& 0\% [\text{\sffamily X}]	& $-3.7$ [\text{\sffamily X}]	& 1.7\% \\
303.01	& $-32.3$ [\text{\sffamily X}]	& 54\% [\checkmark]			& $-1.8$ [\text{\sffamily X}]	& 2.3\% \\
1888.01	& $-23.7$ [\text{\sffamily X}]	& 17\% [\text{\sffamily X}]	& $+0.6$ [\checkmark]			& 3.3\% \\
1925.01	& $+93.9$ [\checkmark]			& 41\% [\text{\sffamily X}]	& $-3.0$ [\text{\sffamily X}]	& 5.9\% \\
2728.01	& $+68.9$ [\checkmark]			& 28\% [\text{\sffamily X}]	& $+0.3$ [\checkmark] 			& 4.6\% \\
3220.01	& $-1.2$ [\text{\sffamily X}]	& 40\% [\text{\sffamily X}]	& $-6.9$ [\text{\sffamily X}]	& 0.39\% \\ 
\hline
K1625b & $+3.2$ & N/A & $+1.9$ & N/A \\ [1ex]
\hline\hline %inserts single line
\end{tabular}
\label{tab:models} % is used to refer this table in the text
\end{table*}
